H-alpha and Ca II Infrared Triplet Variations During a Transit of the 23 Myr Planet V1298 Tau c

Young transiting exoplanets (< 100 Myr) provide crucial insight into atmospheric evolution via photoevaporation. However, transmission spectroscopy measurements to determine atmospheric composition and mass loss are challenging due to the activity and prominent stellar disk inhomogeneities present on young stars. We observed a full transit of V1298 Tau c, a 23 Myr, 5.59$R_\oplus$ planet orbiting a young K0-K1.5 solar analogue with GRACES on Gemini-North. We were able to measure the Doppler tomographic signal of V1298 Tau c using the Ca II infrared triplet (IRT) and find a projected obliquity of $\lambda = 5^\circ \pm 15^\circ$. The tomographic signal is only seen in the chromospherically driven core of the Ca II IRT, which may be the result of star-planet interactions. Additionally, we find that excess absorption of the H-alpha line decreases smoothly during the transit. While this could be a tentative detection of hot gas escaping the planet, we find this variation is consistent with similar timescale observations of other young stars that lack transiting planets over similar timescales. We show this variation can also be explained by the presence of starspots with surrounding facular regions. More observations both in- and out-of the transits of V1298 Tau c are required to determine the nature of the Ca II IRT and H-alpha line variations.

==> style.tex <==
% Packages
\usepackage{xifthen}
\usepackage{stackengine}
\usepackage{tabstackengine}
\usepackage{array}
\usepackage{upgreek}
\usepackage[bbgreekl]{mathbbol}
\usepackage{afterpage}
\usepackage[bb=boondox]{mathalpha}

% Shorthand for this paper
\newcommand{\starry}{\textsf{starry}\xspace}
\newcommand{\celerite}{\textsf{celerite}\xspace}
\newcommand{\cpp}{\textsf{C++}\xspace}
\newcommand{\theano}{\textsf{theano}\xspace}
\newcommand{\pymcthree}{\textsf{pymc3}\xspace}
\newcommand{\starryprocess}{\textsf{starry\_process}\xspace}
\newcommand{\Python}{\textsf{Python}\xspace}
\newcommand{\xxx}[1]{{\color{red}#1}}
\newcommand{\quadquad}{\quad\quad\quad\quad}

% Misc. macros
\newcommand{\LMAX}{15\xspace}

% Integrals
\newcommand{\dd}{\ensuremath{\text{d}}}

% Special functions
\newcommand{\sgn}{{\text{sgn}}}
\newcommand{\atantwo}{{\text{arctan2}}}

% Cartesian unit vectors
\newcommand{\xhat}{\ensuremath{\pmb{\hat{x}}}\xspace}
\newcommand{\yhat}{\ensuremath{\pmb{\hat{y}}}\xspace}
\newcommand{\zhat}{\ensuremath{\pmb{\hat{z}}}\xspace}

% Other
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Inverse diagonal dots
\makeatletter
\def\Ddots{\mathinner{\mkern1mu\raise\p@
                \vbox{\kern7\p@\hbox{.}}\mkern2mu
                \raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
\makeatother

% Imaginary unit
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathscr}{U}{mathc}{m}{it}
\DeclareMathOperator{\imag}{\mathscr{i}}

